Global Aspects of Spaces of Vacua

We study "vacuum crossing", which occurs when the vacua of a theory are exchanged as we vary some periodic parameter $\theta$ in a closed loop. We show that vacuum crossing is a useful non-perturbative tool to study strongly-coupled quantum field theories, since finding vacuum crossing in a weakly-coupled regime of the theory can lead to nontrivial consequences in the strongly-coupled regime. We start by discussing a mechanism where vacuum crossing occurs due to an anomaly, and then discuss some applications of vacuum crossing in general. In particular, we argue that vacuum crossing can be used to check IR dualities and to look for emergent IR symmetries.

==> latex_shortcuts.tex <==
\usepackage{hyperref}
\hypersetup{
	colorlinks,
	citecolor=blue,
	filecolor=blue,
	linkcolor=blue,
	urlcolor=blue,
	linktocpage=true
}


%footnote without marker
\newcommand\blfootnote[1]{%
	\begingroup
	\renewcommand*\thefootnote{}\footnote{#1}%
	\addtocounter{footnote}{-1}%
	\endgroup
}

\usepackage{amsmath}
\usepackage{mathptmx}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{cancel}
\usepackage{verbatim}
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}

%BIBLIOGRAPHY
%\usepackage{cite}
\usepackage[backend=bibtex,sorting=none,style=numeric-comp,url=false]{biblatex}

%\usepackage{babel}

%GRAPHICS
\usepackage{graphicx}

%HEADERS AND FOOTERS
\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
\rhead{\runauthor}
\lhead{\slshape \runtitle}
\rfoot{\thepage}


\usepackage[rgb,dvipsnames]{xcolor}
\newcommand\todo[1]{\textcolor{red}{(#1)}}
\newcommand\note[1]{\textcolor{Fuchsia}{(#1)}}

\newcommand{\munu}{{\mu\nu}}
\newcommand{\munurho}{{\mu\nu\rho}}
\newcommand{\dmu}{{\partial_\mu}}
\newcommand{\Dmu}{{\partial^\mu}}
\newcommand{\dnu}{{\partial_\nu}}
\newcommand{\Dnu}{{\partial^\nu}}

\newcommand{\gryb}{\bar{\psi}}
\newcommand{\psib}{\bar{\psi}}
\newcommand\braceto[2]{\overset{#2}{\overbrace{#1}}}

\newcommand\mb[1]{\mathbb{#1}}
\newcommand\mc[1]{\mathcal{#1}}
\newcommand{\tr}{\text{Tr}}

%GREEK LETTERS
\newcommand{\gra}{\alpha}
\newcommand{\grA}{\Alpha}
\newcommand{\grb}{\beta}
\newcommand{\grB}{\Beta}
\newcommand{\grg}{\gamma}
\newcommand{\grG}{\Gamma}
\newcommand{\grd}{\delta}
\newcommand{\grD}{\Delta}
\newcommand{\gre}{\epsilon}
\newcommand{\grj}{\varphi}
\newcommand{\grf}{\phi}
\newcommand{\grF}{\Phi}
\newcommand{\grt}{\tau}
\newcommand{\grl}{\lambda}
\newcommand{\grL}{\Lambda}
\newcommand{\grs}{\sigma}
\newcommand{\grS}{\Sigma}
\newcommand{\grr}{\rho}
\newcommand{\grn}{\nu}
\newcommand{\grh}{\eta}
\newcommand{\gry}{\psi}
\newcommand{\grY}{\Psi}
\newcommand{\grx}{\xi}
\newcommand{\grk}{\kappa}
\newcommand{\grz}{\zeta}
